Pion Elastic Form Factor in a Rather Broad Range of Momentum Transfers from Local-Duality QCD Sum Rule

Revisiting, within QCD sum rules, the relevance of local duality for the pion elastic form factor gives rise to optimism.

==> contribution.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% template for hadron2011 contribution
%
% please do not rename this file
%
% to create document run
%
%     pdflatex hadron2011.tex
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{  % do not remove


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% please define your macros here

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% define title, author, and address
% contribution[short title]{title}{author first name}{author last name}{author address}{author email}{collaboration}
% the short title will appear in the page headers and the TOC of the book of proceedings
% the last two arguments may be left empty
\contribution[Magneto-Acoustic Coupling to Cyanide Reagents]  % short title (optional)
{Magneto-Acoustic Coupling to Cyanide Reagents \\ and Other Chemicals}  % title
{Despina A.}{Reggiano}  % first and last name of author
{Department of Physical Chemistry \\
  Scuola Normale Superiore di Napoli \\
  I-80222 Napoli, ITALY}  % author address
{reggiano@snsn.it}  % author email optional
{on behalf of the PSI Collaboration}  % collaboration (optional)
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% abstract
\abstract{%
  There is evidence that magnetic fields influence a variety of
  aspects of human and animal physiology, but the precise mode of
  action of the magnetic influence is still not understood. We will
  present evidence that mesmeric influence can disrupt the lethal
  action of sodium cyanide (NaCN) when modulated by a sequence of
  high-pitched tones.
}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% main text
% for short contributions sections are optional
\section{Introduction}

Recently, F. A. Mesmer has reported evidence of a profound influence
of magnets on a variety of aspects of human and animal
physiology~\cite{Mesmer}. Numerous authors have claimed to reproduce
certain of the phenomena reported by Mesmer~\cite{diCenzo,Muller}, but
there is little understanding of the precise mode of action of the
magnetic influence. In this article, I will present evidence that
mesmeric influence can disrupt the lethal action of sodium cyanide
(NaCN) when modulated by a sequence of high-pitched tones. After a
description of the phenomenon, I will comment on the implications for
the nature of the magnetic coupling.


\section{Observations}

My observations began when I was called on an emergency basis to aid
two Albanian noblemen, Guglielmo B. and Ferrando di N., who had
ingested the poison in an apparent attempt to commit suicide. (The
facts of the case were rather mysterious, since these young men had
been seen in the harbor earlier in the day, affecting a carefree
attitude. However, this need not concern us here.) The standard remedy
would have been to induce vomiting; however, this would have offended
the sensibilities of two noble ladies present, the daughters of the
duke in whose household this unfortunate incident took place. Thus, I
thought it wise to begin by administering magneto-therapy using the
devices that I had at hand.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% the recommended way to include figures
\begin{figure}[htb]
  \begin{center}
    % please do not add file name extension this makes switching between latex and pdflatex easier
    \includegraphics[width=0.5\textwidth]{example}
    \caption{The magnet used in the Mesmeric studies.}
    \label{fig:magnet}
  \end{center}
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The source of magnetic influence used in this therapy was the simple
iron pole magnet shown in Figure~\ref{fig:magnet}. The device, roughly
the size of human palm, was held three fingers' length away from each
of the patients, while the blood cyanide level was monitored. As this
operator proceeded in silence, only a very small effect on the poison
was observed. In a moment, however, the sisters began to weep and
ululate in the most painful manner. Under this blanket of sound, the
effects of the cyanide reaction were observed to be completely
reversed. Indeed, even before the end of a single session of
treatment, the Albanians were seen to wake from their comas and offer
thanks for their rescue. Some sample blood cyanide levels are reported
in Table~\ref{tab:blood}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% the recommended way to include a LaTeX table
\begin{table}[tb]
  \begin{center}
    \begin{tabular}{lccc}  
      Patient        & Initial level($\mu$g/cc) & w. Magnet & w. Magnet and Sound \\
      \hline
      Guglielmo B.   &                    0.12  &      0.10 &               0.001 \\
      Ferrando di N. &                    0.15  &      0.11 &          $< 0.0005$ \\
    \end{tabular}
    \caption{Blood cyanide levels for the two patients.}
    \label{tab:blood}
  \end{center}
\end{table}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Interpretation}

A description of these observations, obviously based on second-hand
reports, has already been reported by L. da Ponte~\cite{daPonte}. In
his paper, da Ponte attributes the mode of action of the magnetic
force to direct magnetic attraction. This would be implausible with
the relatively small magnet used in this study; thus da Ponte was
forced to propose an absurdly large size for the magnetic device. His
theory does not account for the acoustic influence, which is known not
to be present in magnetic action on inanimate objects. A second
hypothesis would state that the acoustic fields perturb the chemistry
of the cyanide reactions, allowing the reagents to couple
magnetically. As with the first hypothesis, we are skeptical, since
again this phenomenon has no inorganic counterpart. Thus, we are
forced to conclude, with Mesmer, that magnetism couples directly to
the life force, which, as is well known, can be modulated by musical
influences.

In conclusion, we note that the unusual mode of action of magnetism is
only one of many which have been reported in the literature. It is
likely that there are further unusual magnetic phenomena to be
discovered. All studies to date have involved male patients. But it is
likely that the prevailing belief that `women are all the same' would
be overturned in a similar investigation.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% acknowledgements (optional)
\acknowledgements{%
  I am grateful to Don Alfonso d'Alba for certain services essential
  to this investigation. Additional thanks go to the
  $\Phi\Upsilon\Delta$ fraternity.
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% bibliographic items can be constructed using the LaTeX format in SPIRES
% see http://www.slac.stanford.edu/spires/hep/latex.html
% SPIRES will also supply the CITATION line information; please include it
\begin{thebibliography}{99}
  
\bibitem{Mesmer}
  F. A. Mesmer \etal, Proc. Wien. Acad. Sci. {\bf 13}, 1564, 1593 (1762).
  %% CITATION = PWASA,13,1564;%%
  
\bibitem{diCenzo}
  A. L. di Cenzo, Trans. Acad. Ducal.  Milan., {\bf 23}, 2647 (1771).
  %% CITATION = TAADD,23,2647;%%
  
\bibitem{Muller}
  For an exhaustive review of the Prussian literature, see A. D. M\"uller,
  in Workshop on Action at a Distance, F. Eisenschmidt, ed. (Springer,
  Berlin, 1774).

\bibitem{daPonte}
  L. da Ponte, Trans. N. Y. Acad. Sci., {\bf 3}, 27 (1795).
  %% CITATION = TNYAA,3,27;%%

\end{thebibliography}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


}  % do not remove



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../hadron2011.tex"
%%% End: 

